Cubic graphs with no eigenvalues in the interval (-2,0)

We give a complete characterisation of the cubic graphs with no eigenvalues in the interval $(-2,0)$. There is one thin infinite family consisting of a single graph on $6n$ vertices for each $n \geqslant 2$, and five ``sporadic'' graphs, namely the $3$-prism $K_3 \mathbin{\square} K_2$, the complete bipartite graph $K_{3,3}$, the Petersen graph, the dodecahedron and Tutte's $8$-cage. The proof starts by observing that if a cubic graph has no eigenvalues in $(-2,0)$ then its local structure around a girth-cycle is very constrained. Then a separate case analysis for each possible girth shows that these constraints can be satisfied only by the known examples. All but one of these case analyses can be completed by hand, but for girth five there are sufficiently many cases that it is necessary to use a computer for the analysis.

==> voltages.tex <==
We use the concept of voltage graphs [Section 7.4 in Gross and Tucker + citation for eigenvalues of regular voltage assignment over abelian groups].

%% FOR THE CITATION: The following articles have the lifting of eigenvalues for abelian voltage groups; the first one cites the second one as the original source for abelian groups, but there could be an even older paper in the 80s with maybe Cvetkovic? The voltage graph itself is also called a complex gain graph (but I don't know what the cover is called in this situation), and there are also theorems in that field about the spectrum of the covering graph. The statement we want about the spectrum is not in Gross and Tucker, nor Handbook of Graph Theory. 


% @article{DalFioPacSir2021,
% abstract = {We describe, in a very explicit way, a method for determining the spectra and bases of all the corresponding eigenspaces of arbitrary lifts of graphs (regular or not).},
% author = {Dalfó, C. and Fiol, M. A. and Pavlíková, S. and Širáň, J.},
% address = {New York},
% copyright = {The Author(s) 2022},
% issn = {0925-9899},
% journal = {Journal of algebraic combinatorics},
% keywords = {Charts diagrams etc. ; Combinatorial analysis ; Computer science ; Elevators ; Graphic methods ; Hoisting machinery ; Mathematics ; Order ; Ordered algebraic structures},
% language = {eng},
% number = {2},
% pages = {651-672},
% publisher = {Springer US},
% title = {Spectra and eigenspaces of arbitrary lifts of graphs},
% volume = {54},
% year = {2021},
% }

%@article{KwaLee1992,
% author = {Jin Ho Kwak and Jaeun Lee},
% title = {Caracteristics polynomials of some grap bundlesII},
% journal = {Linear and Multilinear Algebra},
% volume = {32},
% number = {1},
% pages = {61--73},
% year = {1992},
% publisher = {Taylor \& Francis},
% doi = {10.1080/03081089208818147},
% URL = { 
%         https://doi.org/10.1080/03081089208818147
% },
% eprint = { 
    
%         https://doi.org/10.1080/03081089208818147
% }
% }

We have a (weighted) graph  $G$ with $3$ vertices; the vertices are $a,b,c$ and the $4$ edges, $E =\{e_1,e_2,e_3,e_4\}$, where 
\begin{itemize}
	\item $e_1$ is a loop on $a$; 
	\item $e_2$ is incident with $\{a,b\}$;
	\item $e_3$ is incident with $\{b,c\}$ and has weight $2$; and 
	\item $e_4$ is incident with $\{a,c\}$. 
\end{itemize}
See Figure \ref{fig:voltages-quotient}. 

\begin{figure}
    \centering
    \includegraphics[width=0.3\linewidth]{voltage-quotient.pdf}
    \qquad 
    \includegraphics[width=0.3\linewidth]{voltage-quotient-cover3.pdf}
    \caption{\textit{Left: } the base graph $G$ with voltage assignments; the unlabelled edges are assigned $1_{C_n}$ and $\gamma$ is a generator of $C_n$.  \textit{Right:} the covering graph with these voltage assignments for $n=3$. }
    \label{fig:voltages-quotient}
\end{figure}


For the purposes of assigning voltages, we consider the weighted digraph $D$ where every edge is replaced with two oppositely oriented digons. Let $\gamma$ be a generating element of $C_n$.  We will consider a regular voltage assignment $\alpha:E\rightarrow C_n$, such that $\alpha(ac) = \gamma$, $\alpha(ca) = \gamma^{-1}$ and all directed edges are mapped the identity element $1_{C_n}$. 

The covering graph $G^{\alpha}$ is the quotient graph $Q_n$. 

Since $C_n$ is abelian, its characters are easy to consider. Let $\omega = e^{2\pi i/n}$ be a primitive $n$th root of unity. We have matrices 
\[
M_j = \pmat{1&1&\omega^{j} \\ 1 & 0 & 2 \\ \omega^{n-j} & 2 & 0 }
\]
for $j = 0,\ldots, n-1$. The $3n$ eigenvalues of the $M_i$s are exactly the set of eigenvalue of the quotient graph. 
The characteristic polynomial of $M_j$ is 
\[
\begin{split}
\phi(M_i,t)	&= t^3 - t^2 - 6t - 2(\omega^{j} + \omega^{n-j}) + 4 \\
	% &= t^3 - t^2 - 6t - 4\cos\left( \frac{2\pi ij}{n} \right) + 4 \\
 	&= t^3 - t^2 - 6t +  4\left(1 - \cos\left( \frac{2\pi ij}{n} \right) \right).  \\
\end{split}
\]
We can write this as 
$
f(t) = t^3 - t^2 - 6t +  4a  = (t + 2)(t - 3)t + 4a.
$
where $ 0 \leq a \leq 2$. 
If $t_0 \in (-2,0)$, then $t+2 > 0$, $t<0$ and $t-3<0$, so 
\[
 (t + 2)(t - 3)t >0 
\]
and, since  $ 0 \leq a \leq 2$, thus  $f(t_0)>0$ on this interval. 

In general, we can do this for any chain of graphs connected in a cycle. Suppose we have graph $G$, which has vertices $s_1, \ldots, s_k$ and $t_1,\ldots, t_k$. Let $H$ be obtained by taking $n$ copies of $G$ and connecting the $s_i$s  to the $t_i$s. This is the covering graph of a voltage graph. See Figure 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.6\linewidth]{voltage-general-cyclic.pdf}
    \caption{Voltages in the general case. }
    \label{fig:voltages-general}
\end{figure}
Again, we let $\omega = e^{2\pi i/n}$ and let $M_j = A(G) + B$, where 
\[
B_{u,v} = \begin{cases}
    \gamma & \text{ if } u = s_i, v = t_i;\\
    \gamma^{-1} & \text{ if } u = t_i, v = s_i; \text{ and,}\\
    0, & \text{otherwise}.
\end{cases}
\]
The eigenvalues of $H$ are the eigenvalues of $M_j$ for $j=0,\ldots, n$.

This could be used to construct other graphs with spectral gaps, but it's hard to say what the gap, if any, will be. Luckily no cyclic voltages assigned to the Petersen graph results in another example (except when assigned to the perfect matching, which results in disjoint copies of the Petersen graph). 
